Long Story Short: Story-level Video Understanding from 20K Short Films

Recent developments in vision-language models have significantly advanced video understanding. Existing datasets and tasks, however, have notable limitations. Most datasets are confined to short videos with limited events and narrow narratives. For example, datasets with instructional and egocentric videos often depict the activities of one person in a single scene. Although existing movie datasets offer richer content, they are often limited to short-term tasks, lack publicly available videos, and frequently encounter data leakage issues given the use of subtitles and other information about commercial movies during LLM pretraining. To address the above limitations, we propose Short-Films 20K (SF20K), the largest publicly available movie dataset. SF20K consists of 20,143 amateur films, amounting to 3,582 hours of video, with an average of 12 minutes per movie. We accompany this dataset with SF20K-Test, a manual, open-ended question answering benchmark. SF20K-Test consists of 95 movies and 979 question-answer pairs. Our extensive analysis of SF20K-Test reveals limited data leakage, emphasizes the need for long-term reasoning, and demonstrates the strong performance of recent VLMs. Finally, we show that instruction tuning on the large-scale dataset substantially improves model performance, paving the way for future progress in long-term video understanding.

==> figures/ablation_study.tex <==
\begin{table}[h!]
    \centering
    \caption{\textbf{Ablation study} results comparing different modalities and temporal windows. The human column shows the difference between model performance and human performance.}
    \label{tab:ablation_study}
    \begin{tabular}{cccccc}
        \toprule
        \multirow{2}{*}{Method} & \multirow{2}{*}{Modality} & \multicolumn{3}{c}{Performance} & \\
        \cmidrule(r){3-5}
         & & Shot-Level & Scene-Level & Movie-Level & Human \\
        \midrule
        \multirow{3}{*}{FrozenBiLM} & Vision & 22.1 & 22.7 & 23.4 & 59.0 \textcolor{darkgreen}{(+35.6)} \\
        & Language & 30.9 & 34.8 & 38.2 & 70.9 \textcolor{darkgreen}{(+32.7)} \\
        & Vision-Language & 30.8 & 34.8 & 38.6 & 89.8 \textcolor{darkgreen}{(+51.2)} \\
        \midrule
        \multirow{3}{*}{LLoVi} & Vision & 32.8 & 34.2 & 30.8 & 59.0 \textcolor{darkgreen}{(+28.2)} \\
        & Language & 38.5 & 51.2 & 64.2 & 70.9 \textcolor{darkgreen}{(+6.7)} \\
        & Vision-Language & 50.1 & 55.4 & 55.6 & 89.8 \textcolor{darkgreen}{(+34.2)} \\
        \bottomrule
    \end{tabular}
\end{table}


==> figures/data_contamination.tex <==
\definecolor{ao(english)}{rgb}{0.0, 0.5, 0.0}
\definecolor{applegreen}{rgb}{0.55, 0.71, 0.0}
\definecolor{darkgreen}{rgb}{0.0, 0.2, 0.13}

\begin{table}[t]
    \centering
    \begin{tabular}{llll}
        \toprule
        Name     & Size         & MovieQA & SFD   \\
        \midrule
        LLaMA-3  & 8B           & 34.5\%  & 22.1\% \textcolor{ao(english)}{(-12.4\%)} \\
                 & 70B          & 51.9\%  & 24.1\% \textcolor{ao(english)}{(-27.8\%)} \\
        \midrule
        Mixtral  & 7B           & 44.1\%  & 28.9\% \textcolor{ao(english)}{(-15.2\%)} \\
                 & 8$\times$7B  & 59.1\%  & 33.5\% \textcolor{ao(english)}{(-25.6\%)} \\
                 & 8$\times$22B & -       & -      \\
        \midrule
        GPT      & 3.5          & 56.7\%  & 26.3\% \textcolor{ao(english)}{(-30.4\%)} \\
                 & 4            & 71.3\%  & 31.5\% \textcolor{ao(english)}{(-39.8\%)} \\
        \midrule
        Claude 3 & Haiku        & 55.4\%  & 28.9\% \textcolor{ao(english)}{(-26.5\%)} \\
                 & Sonnet       & 64.4\%  & 36.0\% \textcolor{ao(english)}{(-28.4\%)} \\
                 & Opus         & -       & -      \\
        \midrule
        Gemini   & 1.0 pro      & -       & -      \\
                 & 1.5 Flash    & -       & -      \\
                 & 1.5 Pro      & -       & -      \\
        \bottomrule
    \end{tabular}
    \caption{\textbf{Data contamination.}}
    \label{data_contamination}
\end{table}


==> figures/data_contamination_plot.tex <==
\begin{figure*}[t]
    \centering
    \begin{minipage}{0.48\textwidth}
        \centering
        \includegraphics[width=\linewidth]{data/dataset_overview.pdf}
        \captionof{figure}{\textbf{Comparison of SF20K-Test to other VQA test datasets.} The circle size indicates the number of QA pairs in each dataset.
        }
        \label{fig:plot_dataset_comparisons}
    \end{minipage}\hfill
    \begin{minipage}{0.5\textwidth}
        \centering
        %\includegraphics[width=\linewidth]{data/data_contamination_with_llama3.pdf}
        \includegraphics[width=\linewidth]{figures/vic_leakage_SF20K.pdf}
        \captionof{figure}{\textbf{Data leakage.} When given \emph{only} the movie title, higher zero-shot accuracy in question-answering by LLMs indicates greater data leakage. LLMs are ranked by MMLU.}
        %  By providing only the movie title to LLMs, higher zero-shot accuracy on question-answering suggests worse data leakage.
        \label{fig:data_contamination_plot}
    \end{minipage}
\end{figure*}

%\input{figures/vic_play_claude}




==> figures/data_contamination_plot_mmlu.tex <==
\begin{figure}[t]
    \centering
    \begin{minipage}{0.48\textwidth}
        \caption{\textbf{LLM accuracy based on movie titles.} Comparison of accuracy across LLMs, highlighting potential data leakage.}
        \label{fig:data_contamination_table}
        \centering
        \begin{tabular}{lrrrr}
            \toprule
            Name & SFD & MovieQA & LVU \\%& MMLU \\
            \midrule
            \multicolumn{4}{c}{Open-source models} \\
            \midrule
            %Gemma 2B & - & - & - \\%& - \\
            Gemma 7B & 20.7 & 21.5 & 52.4 \\%& 53.3 \\
            %LLaMA 3 8B & 22.1 & 34.5 & - \\%& - \\
            %LLaMA 3 70B & 24.1 & 51.9 & - \\%& - \\
            Mistral 7B & 28.9 & 44.1 & 61.4 \\%& 58.4 \\
            Mixtral 8x7B & 33.5 & 55.4 & 70.2 \\%& 70.6 \\
            \midrule
            \multicolumn{4}{c}{Commercial models} \\
            \midrule
            Claude 3 Haiku & 28.9 & 55.4 & 68.5 \\%& 75.2 \\
            Claude 3 Sonnet & 36.0 & 64.4 & 71.0 \\%& 79.0 \\
            GPT-3.5 & 26.3 & 56.7 & 75.0 \\%& 70.0 \\
            GPT-4 & 31.5 & 71.3 & 76.0 \\%& 86.4 \\
            \bottomrule
        \end{tabular}
    \end{minipage}\hfill
    \begin{minipage}{0.48\textwidth}
        \centering
        \includegraphics[width=\linewidth]{data/data_contamination_mmlu.pdf}
        \captionof{figure}{\textbf{Impact of model knowledge on data leakage.}
        Higher MMLU performance results in LLMs memorizing more information about commercial movies.
        }
        \label{fig:data_contamination_plot}
    \end{minipage}
\end{figure}


==> figures/data_contamination_with_lvu.tex <==
\begin{figure}[t]
    \centering
    \begin{tabular}{lllll}
        \toprule
        Name     & Size         & MovieQA & LVU & SFD   \\
        \midrule
        LLaMA-3  & 8B           & 34.5\%  & -   & 22.1\% \textcolor{darkgreen}{(-12.4\%)} \\
                 & 70B          & 51.9\%  & -   & 24.1\% \textcolor{darkgreen}{(-27.8\%)} \\
        \midrule
        Mixtral  & 7B           & 44.1\%  & -   & 28.9\% \textcolor{darkgreen}{(-15.2\%)} \\
                 & 8$\times$7B  & 59.1\%  & -   & 33.5\% \textcolor{darkgreen}{(-25.6\%)} \\
                 % & 8$\times$22B & -       & -   & -      \\ Xi: we do not need this one right?
        \midrule
        GPT      & 3.5          & 56.7\%  & -   & 26.3\% \textcolor{darkgreen}{(-30.4\%)} \\
                 & 4            & 71.3\%  & -   & 31.5\% \textcolor{darkgreen}{(-39.8\%)} \\
        \midrule
        Claude 3 & Haiku        & 55.4\%  & -   & 28.9\% \textcolor{darkgreen}{(-26.5\%)} \\
                 & Sonnet       & 64.4\%  & -   & 36.0\% \textcolor{darkgreen}{(-28.4\%)} \\
                 & Opus         & 71.3\%  & -   & -      \\
        \midrule
        Gemini   & 1.0 pro      & -       & -   & -      \\
                 & 1.5 Flash    & -       & -   & -      \\
                 & 1.5 Pro      & -       & -   & -      \\
        \bottomrule
    \end{tabular}
    \caption{\textbf{Data contamination}}
    \label{table}
\end{figure}


==> figures/dataset_comparison_table_tmp.tex <==
\begin{table}[ht]
    \centering
    \resizebox{\textwidth}{!}{%
        \begin{tabular}{@{}llrrrccccccc@{}}
        \toprule
        \multirow{2}{*}{Dataset} & \multirow{2}{*}{Annotation} & \multirow{2}{*}{\#QA Pairs} & \multirow{2}{*}{Avg. Length (s)} & \multirow{2}{*}{Total Hours} & \multirow{2}{*}{Multimodal} & \multirow{2}{*}{\makecell{Long\\Temporal Window}} & \multirow{2}{*}{\makecell{Not\\Contaminated}} & \multicolumn{4}{c}{QA Type} \\
        \cmidrule(r){9-12}
        & & & & & & & & Setting & Character & Story & Theme \\
        \midrule
        MSRVTT-QA        & Auto   & ?     & 15  & ? & ? & ? & ? & ? & ? & ? & ? \\
        %MSVD-QA          & ?      & ?     & ?   & ? & ? & ? & ? & ? & ? & ? & ? \\
        TGIF-QA          & Auto   & ?     & 3   & ? & ? & ? & ? & ? & ? & ? & ? \\
        How2QA           & Manual & ?     & 60  & ? & ? & ? & ? & ? & ? & ? & ? \\
        NeXT-QA          & Manual & ?     & 44  & ? & ? & ? & ? & ? & ? & ? & ? \\
        %iVQA             & ?      & ?     & ?   & ? & ? & ? & ? & ? & ? & ? & ? \\
        %ActivityNet-QA   & ?      & ?     & ?   & ? & ? & ? & ? & ? & ? & ? & ? \\
        TVQA             & Manual & ?     & 76  & ?   & ? & ? & ? & ? & ? & ? & ? \\
        MovieQA          & Manual & 6,462 & 203 & ?   & ? & ? & ? & ? & ? & ? & ? \\
        MovieChat (test) & Manual & 1,300 & 500 & ?   & ? & ? & ? & ? & ? & ? & ? \\
        Perception Test  & ?      & ?     & 23  & ?   & ? & ? & ? & ? & ? & ? & ? \\
        EgoSchema        & Manual & 5,000 & 180 & 250 & ? & ? & ? & ? & ? & ? & ? \\
        CinePile (test)  & Manual & 4,940 & 160 & ?   & ? & ? & ? & ? & ? & ? & ? \\
        SFD (Ours)       & Manual & 4,885 & 720 & 243 & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark \\
        \bottomrule
        \end{tabular}%
    }
    \caption{\textbf{Comparison of SFD to other videoQA datasets.}}
    \label{dataset_comparison_table}
\end{table}


==> figures/dataset_samples.tex <==
\begin{table}[t]
    \caption{\textbf{Random samples from different movieQA datasets.}}
    \label{movieqa_samples}
    \centering
    \small
    \resizebox{\textwidth}{!}{%
       \begin{tabular}{lll}
          
        \toprule
        \textbf{Dataset} & \textbf{Questions} & \textbf{Answers} \\
        \midrule
        TVQA & What color is Raj sweater when he was talking to Bernadette? & blue and white \\
         & Who walked up when Joey and Jen were getting their mail? & The man that had the picture of the man looking for a hot girl. \\
         & What does the silver statue between Castle and Beckett look like when they are looking out the window for security cameras? & A very tall human. \\
         & What does Howard say is racing to San Francisco when he monologues? & A Signal \\
         & Where does Foreman notice the vomit before saying what do you make of this? & on the floor in the hay \\
        \midrule
        MovieChat & How many characters appear in the scene wear glasses? & Three. \\
         & Is it at daytime or at night time? & It's at night. \\
         & How many people appeared? & Three. \\
         & Are there any plants? & No. \\
         & How many people appeared? & Six. \\
        \midrule
        LVU & What is the way of speaking of the characters? & confronts \\
         & What genre is the movie? & Action-Crime-Adventure \\
         & In which decade was the movie released? & 2000 \\
         & What genre is the movie? & Comedy \\
         & What is the way of speaking of the characters? & explains \\
        \midrule
        MovieQA & Do the man and his son find the thief? & Yes \\
         & What do Adam and Grace do to escape the crocodile? & They climb into a nearby tree \\
         & What does the Order of the Phoenix inform Harry? & The Ministry of Magic does not believe Voldemort has returned \\
         & What is the name of the White Witch? & Jadis \\
         & Who rescues Edmund from the Witch's castle? & Aslan's troops \\
        \midrule
        CinePile & What is a notable change in the character's appearance during the scene? & Flashing a smile \\
         & What does Rudy notice that leads to him opening a door? & Jen is missing \\
         & Where is Jack during the conversation about Iris's true identity? & In bed \\
         & How does the interaction between Val and Jess change throughout the scene? & It becomes more hostile \\
        \midrule
        SFD & How does Nate end up with a night's stay at a five-star hotel? & The shelter receives a donation in the form of a night's stay at a five-star hotel, which they give to Nate. \\
         & Who interrupts Chris' stakeout? & His sister Lottie \\
         & Were Kate and Simon close during their childhood? & Yes, they were formerly close \\
         & Why is Aris going to a special camp? & Aris is going to a special camp as part of reform and punishment for her propensity to lie. \\
         & Where do Kelsey and Martin first catch each other's eye? & At a nightclub. \\
        \bottomrule
        \end{tabular}%
    }
\end{table}


==> figures/generation_pipeline.tex <==
\begin{figure*}[t]
  \centering
  \includegraphics[width=1\linewidth]{data/detail_pipeline.jpg}
  \caption{\textbf{Data generation pipeline of SFD-Test.} For short films with available synopses, we use an LLM to generate Question-Answer Pairs and to create challenging distractors. Both Open-Ended and Multiple-Choice Questions undergo automatic filtering and manual curation. Annotation details, e.g., shots, clip info, face tracks and subtitles are also extracted and included in the SFD dataset.}
  \label{fig:question_generation}
\end{figure*}


==> figures/human_study.tex <==
\begin{table}[h]
    \centering
    \small
    \begin{tabular}{lrrc}
        \toprule
        Method & \% Accuracy \\
        \midrule
        Human (multimodal) & 89.8\% \\
        Human (vision-only)  & 59.0\%\\
        Human (subtitles-only) & 70.9\% \\
        \bottomrule
    \end{tabular}
    \caption{\textbf{Human Study.}}
    \label{tab:human_study}
\end{table}


==> figures/plot_dataset_comparisons.tex <==
\definecolor{ao(english)}{rgb}{0.0, 0.5, 0.0}
\definecolor{applegreen}{rgb}{0.55, 0.71, 0.0}
\definecolor{darkgreen}{rgb}{0.0, 0.2, 0.13}

\begin{figure}[t]
    \centering
    \begin{minipage}{0.55\textwidth}
        \centering
        \begin{tabular}{llll}
            \toprule
            Name     & Size         & MovieQA & SFD   \\
            \midrule
            LLaMA-3  & 8B           & 34.5\%  & 22.1\% \\%\textcolor{ao(english)}{(-12.4\%)} \\
                     & 70B          & 51.9\%  & 24.1\% \\%\textcolor{ao(english)}{(-27.8\%)} \\
            \midrule
            Mixtral  & 7B           & 44.1\%  & 28.9\% \\%\textcolor{ao(english)}{(-15.2\%)} \\
                     & 8$\times$7B  & 59.1\%  & 33.5\%\textcolor{ao(english)}{(-25.6\%)} \\
            %         & 8$\times$22B & -       & -      \\
            \midrule
            GPT      & 3.5          & 56.7\%  & 26.3\% \textcolor{ao(english)}{(-30.4\%)} \\
                     & 4            & 71.3\%  & 31.5\% \textcolor{ao(english)}{(-39.8\%)} \\
            \midrule
            Claude 3 & Haiku        & 55.4\%  & 28.9\% \textcolor{ao(english)}{(-26.5\%)} \\
                     & Sonnet       & 64.4\%  & 36.0\% \textcolor{ao(english)}{(-28.4\%)} \\
            %         & Opus         & -       & -      \\
            %\midrule
            %Gemini   & 1.0 pro      & -       & -      \\
            %         & 1.5 Flash    & -       & -      \\
            %         & 1.5 Pro      & -       & -      \\
            \bottomrule
        \end{tabular}
        \captionof{table}{\textbf{Data contamination results.}}
        \label{data_contamination}
    \end{minipage}\hfill
    \begin{minipage}{0.41\textwidth}
        \centering
        \includegraphics[width=\linewidth]{data/plot_dataset_comparisons.pdf}
        \caption{\textbf{Comparison of SFD to other videoQA datasets.}}
        \label{fig:plot_dataset_comparisons}
    \end{minipage}
\end{figure}


==> figures/sfd_subsets_dep.tex <==
\begin{table}[h!]
    \label{tab:subset_performance}
    \centering
    \resizebox{1.00\columnwidth}{!}{
        \begin{tabular}{lccc}
            \toprule
            Method & SF20K-Test & SF20K-Test-Silent & SF20K-Test-Expert \\
            \midrule
            \rowcolor{gray!20} \multicolumn{4}{l}{\hspace{0.5cm} Open-source models} \\
            Video-LLaVA-7B~\cite{lin2023videollava} & 8.29 & 7.20 & 3.54 \\
            %Llava-Next-Video-7B~\cite{zhang2024video} & 42.7 & & 9.77 \\
            Llava-OneVision-0.5B~\cite{} & 22.6 & 17.6 & 19.5 \\
            Long-Llava-7B~\cite{} & 33.5 & 20.9 & 29.5 \\
            Llava-OneVision-7B~\cite{} & 37.7 & \textbf{29.0} & 29.0 \\
            Llama-3.2-Vision-11B & \underline{47.8} & \textbf{29.0} & \underline{31.0} \\
            Pixtral-12B & \textbf{49.8} & \underline{24.8} & \textbf{33.0} \\
            %LongVA-7B~\cite{zhang2024long} & & & \\
            %Llava-Next-Video-34B~\cite{zhang2024video} & & & \\
            %Llava-OneVision-72B~\cite{} & & & \\
            \rowcolor{gray!20} \multicolumn{4}{l}{\hspace{0.5cm} Commercial models} \\
            %LloVi & 24.7 & - & - \\
            GPT-4o-mini~\cite{achiam2023gpt} & \textbf{\textit{60.0*}} & - & - \\
            %Gemini-1.5-Flash~\cite{} & & & \\
            \bottomrule
        \end{tabular}
    }
    \vspace{-1em}
    \begin{flushleft}
        \footnotesize ${^*}$ indicates that inference is done on only 10\% of the test set to limit costs.
    \end{flushleft}
   
    \caption{\textbf{Zero-shot performances for OEQA on the Silent and Expert subset} using vision-only and vision and language (VL), respectively. For comparison, we also report the performance on SF20K-Test. \vicc{it is very unclear. since silent movies have only V }
    }
     \label{sfd_subsets}
\end{table}


==> figures/table_data_cont.tex <==
\begin{wraptable}{r}{0.6\textwidth}
    \caption{
    \textbf{LLM accuracy based on movie titles.} Comparison of accuracy across LLMs, highlighting potential data leakage.
    }
    \footnotesize
    \label{fig:data_contamination_table}
    \centering
    \begin{tabular}{lccccc}
        \toprule
        Name & MMLU & SFD & MovieQA & LVU \\
        \midrule
        Gemma 2B & 42.3 & 19.7 & 18.3 & 28.8 \\
        Gemma 7B & 54.3 & 20.7 & 21.5 & 52.4 \\
        Mistral 7B & 62.5 & 28.9 & 44.1 & 69.9 \\
        LLaMA 3 8B & 68.4 & 22.1 & 34.5 & 64.1 \\
        GPT-3.5 & 70.0 & 26.3 & 56.7 & 75.0 \\
        Mixtral 8x7B & 70.6 & 33.5 & 55.4 & 70.2 \\
        Claude 3 Haiku & 75.2 & 28.9 & 55.4 & 68.5 \\
        Claude 3 Sonnet & 79.0 & 36.0 & 64.4 & 71.0 \\
        LLaMA 3 70B & 82.0 & 24.1 & 51.9 & 64.1\\
        GPT-4 & 86.4 & 31.5 & 71.3 & 76.0 \\
        \bottomrule
    \end{tabular}
\end{wraptable}


==> figures/teaser.tex <==
\begin{figure*}[!htbp]
% \vspace{-8mm}
    %\includegraphics[width=0.99\linewidth]{data/Finalteaser_xi11.jpg}
    \includegraphics[width=1.0\linewidth]{figures/vic_teaser_SF20K.pdf}
    % if you like this, you can download the pptx from here: 
    % https://www.dropbox.com/scl/fi/ye1c9a5yk47osr4w2pxtd/vic_teaser.pptx?rlkey=5sn4na2cz18f1ju9xla4ejpts&dl=0
    % and change it accordingly. I cannot upload it as it's too big. 
    % \vspace{-5mm}
    \caption{\small \textbf{VideoQA examples from three video domains: instructional videos, egocentric videos and movies.} While instructional and egocentric videos usually depict one or two people performing a single task, movies present time-extended stories with rich variety in terms of scenes, characters and interactions. 
    % \vicc{move the Question from everywhere a bit to the left so that it doesn't take more than two rows in the second subfigure (egocentric);}
    % \vicc{move the Answer from everywhere a bit to the left so that it doesn't take more than two rows in the last subfigure (ours)} \vicc{SFD (ours) is not very visible; make it more?}
    %\vspace{-7mm} 
    \vicc{make this prettier please!}
   }
  %\vicc{here, perhaps it would make sense to change it as follows: 
  %  think of a table with four rows and two columns (we won't have a table, but to give you the idea). 
  %  The first row corresponds to instructional videos
  %  the second to egocentric 
  %  the third to movie, specifically choose one (eg MovieQA) 
  %  the fourth one to SDF. 
  %  Below each set of examples we also have one Q\&A Pair. 
  %  On the right side of the table we have list of items with crosses and checkmarks for each domain. 
  % (1) `story': for rows 1, 2 we have a cross, whereas for rows 3,4 we have checkmark
  % (2) character information: for rows 1, 2 we have a cross, whereas for rows 3,4 we have checkmark 
  % (3) copyrights: rows 1, 2, 4 checkmarks, row 3 cross 
  % (4) not contaminated: rows 1, 2, 4 checkmarks, row 3 cross (here we can highlight something in the Q\&A that we will have below each set of examples for each domain 
  % (5) long term reasoning: this is tricky 
  % (6) complex story line.  
  % What do you think? If yes, do not forget to write in the caption what each item on the right represents (especially for this contaminated term)}}
    \label{fig:teaser}
\end{figure*}

% \begin{figure}[h]
%     \includegraphics[width=1\linewidth]{data/teaser.pdf}
%     \caption{\textbf{Example frames from three video domains: movies, instructional videos, and egocentric videos.} While instructional and egocentric videos usually depict a single person performing one task, movies exhibit a large variety of camera poses, scene configurations, characters and interactions. }
%     \label{fig:teaser}
% \end{figure}



==> sections/supmat/checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Checklist}
\label{subsec:checklist}
\begin{comment}
%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%
\end{comment}

% \begin{enumerate}

% \item For all authors...
% \begin{enumerate}
%   \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
%     \answerYes{}
%   \item Did you describe the limitations of your work?
%     \answerYes{}
%   \item Did you discuss any potential negative societal impacts of your work?
%     \answerYes{See Supplementary Materials Section~\ref{subsec:ethical_considerations}}
%   \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
%     \answerYes{See Supplementary Materials Section~\ref{subsec:ethical_considerations}}
% \end{enumerate}

% \item If you are including theoretical results...
% \begin{enumerate}
%   \item Did you state the full set of assumptions of all theoretical results?
%     \answerNA{}
% 	\item Did you include complete proofs of all theoretical results?
%     \answerNA{}
% \end{enumerate}

% \item If you ran experiments (e.g. for benchmarks)...
% \begin{enumerate}
%   \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
%     \answerYes{~\url{https://huggingface.co/datasets/rghermi/sfd}}
%   \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
%     \answerYes{See Sections~\ref{subsec:baselines}, ~\ref{subsec:temporal_window_study}, and ~\ref{subsec:data_leakage}.}
% 	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
%     \answerNo{} Our experiments consist of benchmarking various aspects of our dataset. For a given compute, instead of performing one experiment several times (with different random seeds), we chose to experiment with several different multimodal methods and multiple LLMs. We observed that they all report similar performances and overall follow the same trend; hence, we argue that our findings are generalizable.
% 	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
%     \answerYes{See Section~3.3}
% \end{enumerate}

% \item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
% \begin{enumerate}
%   \item If your work uses existing assets, did you cite the creators?
%     \answerYes{See Section~\ref{subsec:ethical_considerations}.}
%   \item Did you mention the license of the assets?
%     \answerYes{See Section~\ref{subsec:ethical_considerations}.}
%   \item Did you include any new assets either in the supplemental material or as a URL?
%     \answerNA{}
%   \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
%     \answerYes{See Section~\ref{subsec:ethical_considerations}.}
%   \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
%     \answerNA{
%     %See Section~\ref{subsec:ethical_considerations}.}%\XWC{do we really discuss this?
%     }
% \end{enumerate}

% \item If you used crowdsourcing or conducted research with human subjects...
% \begin{enumerate}
%   \item Did you include the full text of instructions given to participants and screenshots, if applicable?
%     \answerYes{See Section~\ref{subsec:human_study}.}
%   \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
%     \answerNA{}
%   \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
%     \answerNA{}
% \end{enumerate}

% \end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> sections/supmat/instruction_tuning_add_results.tex <==
\begin{comment}
\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{data/it_size_ablation.pdf}
    \caption{\textbf{Effect of the training size on the instruction tuning of Llava-OneVision-0.5B trained on Multiple-Choice QA.} Note that the number of instruction samples is approximately 10x the number of videos.}
    \label{fig:it_size_ablation}
\end{figure}

\section{Instruction tuning additional results}
\label{subsec:instruction_tuning_add_results}

We report additional results from the instruction tuning experiment detailed in Section~4.6.

\noindent\textbf{Effect of the training size.} Figure~\ref{fig:it_size_ablation} shows the performance of Llava-OneVision-0.5B~\cite{li2024llavaonevisioneasyvisualtask} when instruction-tuned for multiple-choice question answering on SF20K-Train, with varying numbers of training videos. We subsample the full dataset at incremental values (70, 140, 281, 562, 1125, 2250, 4500, 9000, and 18,000 videos). Results indicate a logarithmic improvement in accuracy as the training set size increases, rising from 46.5\% to 63.0\%. Results are displayed in log-scale. These findings highlight the scalability benefits of instruction tuning on SF20K.

\noindent\textbf{Open-ended QA performance.} Table~\ref{tab:oeqa_it_perf} shows Llava-OneVision-0.5B~\cite{li2024llavaonevisioneasyvisualtask} performance on open-ended question answering after instruction tuning. 
%In details, we unify both multiple-choice and open-ended QA using a similar response format: "(X) [RESPONSE]" for multiple-choice QA and "[RESPONSE]".
Despite the being a much more complex task, we observe a modest overall improvement of +4.0\%.
\end{comment}

\begin{comment}
\begin{table}
    \label{}
    \centering
    \resizebox{1.0\columnwidth}{!}{
    \begin{tabular}{crcccc}
        \toprule
        \multirow{2}{*}{Fine-tuned} & \multirow{2}{*}{\#Videos} & \multicolumn{2}{c}{Multiple-Choice QA} & \multicolumn{2}{c}{Open-Ended QA} \\
        & & VL & $+\Delta$ & VL & $+\Delta$ \\
        \midrule
        \rxmark &      - & 37.8 & & 22.6 & \\
        \gcmark &     70 & 46.5 & \textcolor{my_green}{+8.7} & x & \textcolor{my_green}{+x} \\
        \gcmark &    140 & 49.6 & \textcolor{my_green}{+11.8} & x & \textcolor{my_green}{+x} \\
        \gcmark &    281 & 56.1 & \textcolor{my_green}{+18.3} & x & \textcolor{my_green}{+x} \\
        \gcmark &    562 & 58.5 & \textcolor{my_green}{+20.7} & x & \textcolor{my_green}{+x} \\
        \gcmark &  1,125 & 59.4 & \textcolor{my_green}{+21.6} & x & \textcolor{my_green}{+x} \\
        \gcmark &  2,250 & 60.0 & \textcolor{my_green}{+22.2} & x & \textcolor{my_green}{+x} \\
        \gcmark &  4,500 & 61.1 & \textcolor{my_green}{+23.3} & x & \textcolor{my_green}{+x} \\
        \gcmark &  9,000 & 61.1 & \textcolor{my_green}{+23.3} & x & \textcolor{my_green}{+x} \\
        \gcmark & 18,000 & 63.0 & \textcolor{my_green}{+25.2} & x & \textcolor{my_green}{+x} \\
        \bottomrule
    \end{tabular}
    }
    \caption{Llava-OneVision-0.5B}
\end{table}
\end{comment}

\begin{comment}
\begin{table}
    \label{}
    \centering
    \resizebox{1.0\columnwidth}{!}{
    \begin{tabular}{crcc}
        \toprule
        \multirow{2}{*}{Fine-tuned} & \multirow{2}{*}{\#Videos} & \multicolumn{2}{c}{Multiple-Choice QA} \\
        & & VL & $+\Delta$ \\
        \midrule
        \rxmark &      - & 37.8 & \\
        \gcmark &     70 & 46.5 & \textcolor{my_green}{+8.7} \\
        \gcmark &    140 & 49.6 & \textcolor{my_green}{+11.8} \\
        \gcmark &    281 & 56.1 & \textcolor{my_green}{+18.3} \\
        \gcmark &    562 & 58.5 & \textcolor{my_green}{+20.7} \\
        \gcmark &  1,125 & 59.4 & \textcolor{my_green}{+21.6} \\
        \gcmark &  2,250 & 60.0 & \textcolor{my_green}{+22.2} \\
        \gcmark &  4,500 & 61.1 & \textcolor{my_green}{+23.3} \\
        \gcmark &  9,000 & 61.1 & \textcolor{my_green}{+23.3} \\
        \gcmark & 18,000 & 63.0 & \textcolor{my_green}{+25.2} \\
        \bottomrule
    \end{tabular}
    }
    \caption{Llava-OneVision-0.5B}
\end{table}
\end{comment}

